Large Language Models Can Be Strong Differentially Private Learners

Differentially Private (DP) learning has seen limited success for building large deep learning models of text, and straightforward attempts at applying Differentially Private Stochastic Gradient Descent (DP-SGD) to NLP tasks have resulted in large performance drops and high computational overhead. We show that this performance drop can be mitigated with (1) the use of large pretrained language models; (2) non-standard hyperparameters that suit DP optimization; and (3) fine-tuning objectives which are aligned with the pretraining procedure. With the above, we obtain NLP models that outperform state-of-the-art DP-trained models under the same privacy budget and strong non-private baselines -- by directly fine-tuning pretrained models with DP optimization on moderately-sized corpora. To address the computational challenge of running DP-SGD with large Transformers, we propose a memory saving technique that allows clipping in DP-SGD to run without instantiating per-example gradients for any linear layer in the model. The technique enables privately training Transformers with almost the same memory cost as non-private training at a modest run-time overhead. Contrary to conventional wisdom that DP optimization fails at learning high-dimensional models (due to noise that scales with dimension) empirical results reveal that private learning with pretrained language models doesn't tend to suffer from dimension-dependent performance degradation. Code to reproduce results can be found at https://github.com/lxuechen/private-transformers.

==> Makefile <==
TEXTIDOTE_VERSION := $(shell textidote --version 2>/dev/null)
IGNORE_RULES="sh:c:noin,lt:en:MORFOLOGIK_RULE_EN_US,lt:en:EN_UNPAIRED_BRACKETS,lt:en:CURRENCY,lt:en:PUNCTUATION_PARAGRAPH_END,sh:seclen"

main.pdf: clean
	latexmk -pdf main 2>&1 | awk 'BEGIN{IGNORECASE=1}/warning|!/,/^$$/;'

update:
	cd tex-common && git pull

clean:
	rm main.pdf *.aux *.bbl *.blg *.dvi *.fdb_latexmk *.fls *.log || true

linter:
	chktex -l .chktexrc -V  main.tex

spell:
	./.githooks/spelling.sh .

textidote.jar:
	wget "https://github.com/sylvainhalle/textidote/releases/download/v0.8.1/textidote.jar"

style: textidote.jar
	java -jar textidote.jar --check en --ignore ${IGNORE_RULES} --output singleline main.tex

fullstyle: textidote.jar
	java -jar textidote.jar --check en --ignore ${IGNORE_RULES} --output plain main.tex

emacs:
	emacs --batch -l ~/.emacs --eval "(TeX-auto-generate \"tex-common/macros.sty\" \"auto\")"

makereview:
	git checkout -b reviewed && git push --set-upstream origin reviewed

default:
	pdflatex main
	bibtex main

